ReWiS: Reliable Wi-Fi Sensing Through Few-Shot Multi-Antenna Multi-Receiver CSI Learning

Thanks to the ubiquitousness of Wi-Fi access points and devices, Wi-Fi sensing enables transformative applications in remote health care, security, and surveillance. Existing work has explored the usage of machine learning on channel state information (CSI) computed from Wi-Fi packets to classify events of interest. However, most of these algorithms require a significant amount of data collection, as well as extensive computational power for additional CSI feature extraction. Moreover, the majority of these models suffer from poor accuracy when tested in a new/untrained environment. In this paper, we propose ReWiS, a novel framework for robust and environment-independent Wi-Fi sensing. The key innovation of ReWiS is to leverage few-shot learning (FSL) as the inference engine, which (i) reduces the need for extensive data collection and application-specific feature extraction; (ii) can rapidly generalize to new tasks by leveraging only a few new samples. We prototype ReWiS using off-the-shelf Wi-Fi equipment and showcase its performance by considering a compelling use case of human activity recognition. Thus, we perform an extensive data collection campaign in three different propagation environments with two human subjects. We evaluate the impact of each diversity component on the performance and compare ReWiS with a traditional convolutional neural network (CNN) approach. Experimental results show that ReWiS improves the performance by about 40% with respect to existing single-antenna low-resolution approaches. Moreover, when compared to a CNN-based approach, ReWiS shows a 35% more accuracy and less than 10% drop in accuracy when tested in different environments, while the CNN drops by more than 45%.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> tex_files/CM_CNN_vs_proposed/A1/CNN_1x1_A1.tex <==
\begin{tikzpicture}
\pgfplotsset{every tick label/.append style={font=\tiny}}

\begin{axis}[
enlargelimits=false,
colorbar,
colormap/Purples,
width=\fwidth,
height=\fheight,
at={(0\fwidth,0\fheight)},
scale only axis,
tick align=inside,
xlabel={actual activity},
xmin=-0.5,
xmax=3.5,
xtick style={draw=none},
xlabel style={font=\scriptsize\color{white!15!black}},
ylabel style={font=\scriptsize\color{white!15!black}},
ylabel={predicted activity},
ymin=-0.5,
ymax=3.5,
xlabel shift=-5pt,
ylabel shift=-5pt,
xticklabels={empty, jump, stand, walk},
xtick={0,1,2,3},
% xticklabel style={anchor=center},
ytick={0,1,2,3},
yticklabels={empty, jump, stand, walk},
ytick style={draw=none},
axis background/.style={fill=white},
colorbar horizontal,
colorbar style={
at={(0,1.05)},               % <-- (changed)
anchor=below south west,    % <-- (changed)
% change the width of the colorbar relative to the main `axis' environment
width=\pgfkeysvalueof{/pgfplots/parent axis width},
xtick={0, 0.5, 1},
xmin=0,
xmax=1,
axis x line*=top,
xticklabel shift=-1pt,
point meta min=0,
point meta max=1,
},
% Bottom nodes 
% #1: the THRESHOLD after which we switch to a special display.
nodes near coords bottom/.style={
    % a new feature since 1.9: allows to place markers absolutely:
    scatter/position=absolute,
    close to zero/.style={at={(axis cs:\pgfkeysvalueof{/data point/x},\pgfkeysvalueof{/data point/y})}, xshift=0pt, yshift=-5pt, black, font=\tiny,
    /pgf/number format/.cd,
    fixed,
    fixed zerofill,
    precision=2,
    /tikz/.cd
    },
    big value/.style={at={(axis cs:\pgfkeysvalueof{/data point/x},\pgfkeysvalueof{/data point/y})}, xshift=0pt, yshift=-5pt, white, font=\tiny,
    /pgf/number format/.cd,
    fixed,
    fixed zerofill,
    precision=2,
    /tikz/.cd
    },
    every node near coord/.style={
      check for zero/.code={%
        \pgfmathfloatifflags{\pgfplotspointmeta}{0}{%
            % If meta=0, make the node a coordinate (which doesn't have text)
            \pgfkeys{/tikz/coordinate}%
        }{%
            \begingroup
            % this group is merely to switch to FPU locally. Might be
            % unnecessary, but who knows.
            \pgfkeys{/pgf/fpu}%
            \pgfmathparse{\pgfplotspointmeta<#1}%
            \global\let\result=\pgfmathresult
            \endgroup
            %
            % simplifies debugging:
            %\show\result
            %
            \pgfmathfloatcreate{1}{1.0}{0}%
            \let\ONE=\pgfmathresult
            \ifx\result\ONE
                % AH : our condition 'y < #1' is met.
                \pgfkeysalso{/pgfplots/close to zero}%
            \else
                % ok, proceed as usual.
                \pgfkeysalso{/pgfplots/big value}%
            \fi
        }
      },
      check for zero, 
      % font=\footnotesize, 
      % rotate=90, anchor=west,
    },%
},%
nodes near coords bottom=0.5,
colorbar/width=2mm,
nodes near coords={\pgfmathprintnumber\pgfplotspointmeta},
]
\addplot [matrix plot,point meta=explicit]
 coordinates {
(0,0) [1] (0,1) [0.0001] (0,2) [0.1] (0,3) [0.0001] 

(1,0) [0.0001] (1,1) [1] (1,2) [0.1] (1,3) [0.0001] 

(2,0) [0.00001] (2,1) [0.0001] (2,2) [0.3] (2,3) [0.0001] 

(3,0) [0.0001] (3,1) [0.0001] (3,2) [0.5] (3,3) [1] 
};
\end{axis}
\end{tikzpicture}

% CF:  [[1.  0.  0.  0. ]
%  [0.  1.  0.  0. ]
%  [0.1 0.1  0.3 0.5]
%  [0.  0.  0.  1. ]]


% 12 beam CB, L = 1
%
%        TM0    TM1    JJ0     JJ1
% TM0   81.02  18.94  11.90   29.20
% TM1   25.13  86.63  41.40   26.35            
% JJ0   11.81  26.54  84.01   47.50
% JJ1   24.78  32.16  39.18   80.67
%
%       Train(x), Test(y)

% Average 83.08\% 

% 18.94  + 11.90  + 29.20 + 25.13 + 41.40 +  26.35    + 11.81  +  26.54 +  47.50 + 24.78 + 32.16 +  39.18 /  12 = 27.90

% 12 beam CB, L = 5
%
%        TM0    TM1    JJ0     JJ1
% TM0   84.02  25.91  9.74    15.77
% TM1   21.56  92.43  40.93   20.06                
% JJ0   11.02  17.11  91.89   45.20
% JJ1   20.84  28.89  46.45   91.27

% (84.02 + 92.43 + 91.89 + 91.27) / 4 = 89.90
%(25.91  + 9.74  +  15.77 +  21.56 + 40.93 +  20.06  +  11.02  17.11 +  45.20 + 20.84 + 28.89 + 46.45)/12 = 25.29

==> tex_files/CM_CNN_vs_proposed/A1/CNN_1x4_A1.tex <==
\begin{tikzpicture}
\pgfplotsset{every tick label/.append style={font=\tiny}}

\begin{axis}[
enlargelimits=false,
colorbar,
colormap/Purples,
width=\fwidth,
height=\fheight,
at={(0\fwidth,0\fheight)},
scale only axis,
tick align=inside,
xlabel={actual activity},
xmin=-0.5,
xmax=3.5,
xtick style={draw=none},
xlabel style={font=\scriptsize\color{white!15!black}},
ylabel style={font=\scriptsize\color{white!15!black}},
ylabel={predicted activity},
ymin=-0.5,
ymax=3.5,
xlabel shift=-5pt,
ylabel shift=-5pt,
xticklabels={empty, jump, stand, walk},
xtick={0,1,2,3},
% xticklabel style={anchor=center},
ytick={0,1,2,3},
yticklabels={empty, jump, stand, walk},
ytick style={draw=none},
axis background/.style={fill=white},
colorbar horizontal,
colorbar style={
at={(0,1.05)},               % <-- (changed)
anchor=below south west,    % <-- (changed)
% change the width of the colorbar relative to the main `axis' environment
width=\pgfkeysvalueof{/pgfplots/parent axis width},
xtick={0, 0.5, 1},
xmin=0,
xmax=1,
axis x line*=top,
xticklabel shift=-1pt,
point meta min=0,
point meta max=1,
},
% Bottom nodes 
% #1: the THRESHOLD after which we switch to a special display.
nodes near coords bottom/.style={
    % a new feature since 1.9: allows to place markers absolutely:
    scatter/position=absolute,
    close to zero/.style={at={(axis cs:\pgfkeysvalueof{/data point/x},\pgfkeysvalueof{/data point/y})}, xshift=0pt, yshift=-5pt, black, font=\tiny,
    /pgf/number format/.cd,
    fixed,
    fixed zerofill,
    precision=2,
    /tikz/.cd
    },
    big value/.style={at={(axis cs:\pgfkeysvalueof{/data point/x},\pgfkeysvalueof{/data point/y})}, xshift=0pt, yshift=-5pt, white, font=\tiny,
    /pgf/number format/.cd,
    fixed,
    fixed zerofill,
    precision=2,
    /tikz/.cd
    },
    every node near coord/.style={
      check for zero/.code={%
        \pgfmathfloatifflags{\pgfplotspointmeta}{0}{%
            % If meta=0, make the node a coordinate (which doesn't have text)
            \pgfkeys{/tikz/coordinate}%
        }{%
            \begingroup
            % this group is merely to switch to FPU locally. Might be
            % unnecessary, but who knows.
            \pgfkeys{/pgf/fpu}%
            \pgfmathparse{\pgfplotspointmeta<#1}%
            \global\let\result=\pgfmathresult
            \endgroup
            %
            % simplifies debugging:
            %\show\result
            %
            \pgfmathfloatcreate{1}{1.0}{0}%
            \let\ONE=\pgfmathresult
            \ifx\result\ONE
                % AH : our condition 'y < #1' is met.
                \pgfkeysalso{/pgfplots/close to zero}%
            \else
                % ok, proceed as usual.
                \pgfkeysalso{/pgfplots/big value}%
            \fi
        }
      },
      check for zero, 
      % font=\footnotesize, 
      % rotate=90, anchor=west,
    },%
},%
nodes near coords bottom=0.5,
colorbar/width=2mm,
nodes near coords={\pgfmathprintnumber\pgfplotspointmeta},
]
\addplot [matrix plot,point meta=explicit]
 coordinates {
(0,0) [1] (0,1) [0.0001] (0,2) [0.0001] (0,3) [0.0001] 

(1,0) [0.0001] (1,1) [1] (1,2) [0.0001] (1,3) [0.0001] 

(2,0) [0.00001] (2,1) [0.0001] (2,2) [0.3] (2,3) [0.0001] 

(3,0) [0.0001] (3,1) [0.0001] (3,2) [0.7] (3,3) [1] 
};
\end{axis}
\end{tikzpicture}

% CF:  [[1.  0.  0.  0. ]
%  [0.  1.  0.  0. ]
%  [0.  0.  0.3 0.7]
%  [0.  0.  0.  1. ]]


% 12 beam CB, L = 1
%
%        TM0    TM1    JJ0     JJ1
% TM0   81.02  18.94  11.90   29.20
% TM1   25.13  86.63  41.40   26.35            
% JJ0   11.81  26.54  84.01   47.50
% JJ1   24.78  32.16  39.18   80.67
%
%       Train(x), Test(y)

% Average 83.08\% 

% 18.94  + 11.90  + 29.20 + 25.13 + 41.40 +  26.35    + 11.81  +  26.54 +  47.50 + 24.78 + 32.16 +  39.18 /  12 = 27.90

% 12 beam CB, L = 5
%
%        TM0    TM1    JJ0     JJ1
% TM0   84.02  25.91  9.74    15.77
% TM1   21.56  92.43  40.93   20.06                
% JJ0   11.02  17.11  91.89   45.20
% JJ1   20.84  28.89  46.45   91.27

% (84.02 + 92.43 + 91.89 + 91.27) / 4 = 89.90
%(25.91  + 9.74  +  15.77 +  21.56 + 40.93 +  20.06  +  11.02  17.11 +  45.20 + 20.84 + 28.89 + 46.45)/12 = 25.29

==> tex_files/CM_CNN_vs_proposed/A1/CNN_3x1_A1.tex <==
\begin{tikzpicture}
\pgfplotsset{every tick label/.append style={font=\tiny}}

\begin{axis}[
enlargelimits=false,
colorbar,
colormap/Purples,
width=\fwidth,
height=\fheight,
at={(0\fwidth,0\fheight)},
scale only axis,
tick align=inside,
xlabel={actual activity},
xmin=-0.5,
xmax=3.5,
xtick style={draw=none},
xlabel style={font=\scriptsize\color{white!15!black}},
ylabel style={font=\scriptsize\color{white!15!black}},
ylabel={predicted activity},
ymin=-0.5,
ymax=3.5,
xlabel shift=-5pt,
ylabel shift=-5pt,
xticklabels={empty, jump, stand, walk},
xtick={0,1,2,3},
% xticklabel style={anchor=center},
ytick={0,1,2,3},
yticklabels={empty, jump, stand, walk},
ytick style={draw=none},
axis background/.style={fill=white},
colorbar horizontal,
colorbar style={
at={(0,1.05)},               % <-- (changed)
anchor=below south west,    % <-- (changed)
% change the width of the colorbar relative to the main `axis' environment
width=\pgfkeysvalueof{/pgfplots/parent axis width},
xtick={0, 0.5, 1},
xmin=0,
xmax=1,
axis x line*=top,
xticklabel shift=-1pt,
point meta min=0,
point meta max=1,
},
% Bottom nodes 
% #1: the THRESHOLD after which we switch to a special display.
nodes near coords bottom/.style={
    % a new feature since 1.9: allows to place markers absolutely:
    scatter/position=absolute,
    close to zero/.style={at={(axis cs:\pgfkeysvalueof{/data point/x},\pgfkeysvalueof{/data point/y})}, xshift=0pt, yshift=-5pt, black, font=\tiny,
    /pgf/number format/.cd,
    fixed,
    fixed zerofill,
    precision=2,
    /tikz/.cd
    },
    big value/.style={at={(axis cs:\pgfkeysvalueof{/data point/x},\pgfkeysvalueof{/data point/y})}, xshift=0pt, yshift=-5pt, white, font=\tiny,
    /pgf/number format/.cd,
    fixed,
    fixed zerofill,
    precision=2,
    /tikz/.cd
    },
    every node near coord/.style={
      check for zero/.code={%
        \pgfmathfloatifflags{\pgfplotspointmeta}{0}{%
            % If meta=0, make the node a coordinate (which doesn't have text)
            \pgfkeys{/tikz/coordinate}%
        }{%
            \begingroup
            % this group is merely to switch to FPU locally. Might be
            % unnecessary, but who knows.
            \pgfkeys{/pgf/fpu}%
            \pgfmathparse{\pgfplotspointmeta<#1}%
            \global\let\result=\pgfmathresult
            \endgroup
            %
            % simplifies debugging:
            %\show\result
            %
            \pgfmathfloatcreate{1}{1.0}{0}%
            \let\ONE=\pgfmathresult
            \ifx\result\ONE
                % AH : our condition 'y < #1' is met.
                \pgfkeysalso{/pgfplots/close to zero}%
            \else
                % ok, proceed as usual.
                \pgfkeysalso{/pgfplots/big value}%
            \fi
        }
      },
      check for zero, 
      % font=\footnotesize, 
      % rotate=90, anchor=west,
    },%
},%
nodes near coords bottom=0.5,
colorbar/width=2mm,
nodes near coords={\pgfmathprintnumber\pgfplotspointmeta},
]
\addplot [matrix plot,point meta=explicit]
 coordinates {
(0,0) [1] (0,1) [0.0001] (0,2) [0.1] (0,3) [0.0001] 

(1,0) [0.0001] (1,1) [1] (1,2) [0.1] (1,3) [0.0001] 

(2,0) [0.00001] (2,1) [0.0001] (2,2) [0.3] (2,3) [0.0001] 

(3,0) [0.0001] (3,1) [0.0001] (3,2) [0.5] (3,3) [1] 
};
\end{axis}
\end{tikzpicture}

% CF:  [[1.  0.  0.  0. ]
%  [0.  1.  0.  0. ]
%  [0.1 0.1  0.3 0.5]
%  [0.  0.  0.  1. ]]


% 12 beam CB, L = 1
%
%        TM0    TM1    JJ0     JJ1
% TM0   81.02  18.94  11.90   29.20
% TM1   25.13  86.63  41.40   26.35            
% JJ0   11.81  26.54  84.01   47.50
% JJ1   24.78  32.16  39.18   80.67
%
%       Train(x), Test(y)

% Average 83.08\% 

% 18.94  + 11.90  + 29.20 + 25.13 + 41.40 +  26.35    + 11.81  +  26.54 +  47.50 + 24.78 + 32.16 +  39.18 /  12 = 27.90

% 12 beam CB, L = 5
%
%        TM0    TM1    JJ0     JJ1
% TM0   84.02  25.91  9.74    15.77
% TM1   21.56  92.43  40.93   20.06                
% JJ0   11.02  17.11  91.89   45.20
% JJ1   20.84  28.89  46.45   91.27

% (84.02 + 92.43 + 91.89 + 91.27) / 4 = 89.90
%(25.91  + 9.74  +  15.77 +  21.56 + 40.93 +  20.06  +  11.02  17.11 +  45.20 + 20.84 + 28.89 + 46.45)/12 = 25.29

==> tex_files/figure.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[t]
    \begin{subfigure}[t]{0.23\textwidth}
    \centering
    \setlength\fwidth{.7\textwidth}
    \setlength\fheight{0.4\textwidth}
    \input{./tex_files/CM_CNN_vs_proposed/A1/CNN_1x1_A1}
    \caption{CNN, 1 rx, 1 antenna, $A_1$}
    \label{fig:CM_20_1x1}
    \end{subfigure}
    %
    \hfill
    %
    \begin{subfigure}[t]{0.23\textwidth}
    \centering
    \setlength\fwidth{.7\textwidth}
    \setlength\fheight{0.4\textwidth}
    \input{./tex_files/CM_CNN_vs_proposed/A1/CNN_1x4_A1}
    \caption{CNN, 1 rx, 4 antenna, $A_1$}
    \label{fig:CM_80_1x1}
    \end{subfigure}
     %
    \hfill
    %
    \begin{subfigure}[t]{0.23\textwidth}
    \centering
    \setlength\fwidth{.7\textwidth}
    \setlength\fheight{0.4\textwidth}
    \input{./tex_files/CM_80_1x1}
    \caption{1 \gls{ap}, 1 antenna, 80 MHz}
    \label{fig:CM_80_1x1}
    \end{subfigure}
    %
    \hfill
    %
    \begin{subfigure}[t]{0.23\textwidth}
    \centering
    \setlength\fwidth{.7\textwidth}
    \setlength\fheight{0.4\textwidth}
    \input{./tex_files/CM_80_1x1}
    \caption{1 \gls{ap}, 1 antenna, 80 MHz}
    \label{fig:CM_80_1x1}
    \end{subfigure}
        \setlength\abovecaptionskip{0.2cm}
    \centering
    \begin{subfigure}[t]{0.23\textwidth}
    \centering
    \setlength\fwidth{.7\textwidth}
    \setlength\fheight{0.4\textwidth}
    \input{./tex_files/CM_20_3x4}
    \caption{3 \glspl{ap}, 4 antennas, 20 MHz}
    \label{fig:CM_20_3x4}
    \end{subfigure}
    %
    \hfill
    %
    \begin{subfigure}[t]{0.23\textwidth}
    \centering
    \setlength\fwidth{.7\textwidth}
    \setlength\fheight{0.4\textwidth}
    \input{./tex_files/CM_80_3x4}
    \caption{3 \glspl{ap}, 4 antennas, 80 MHz}
    \label{fig:CM_80_3x4}
    \end{subfigure}
    %
    \hfill
    %
    \begin{subfigure}[t]{0.23\textwidth}
    \centering
    \setlength\fwidth{.7\textwidth}
    \setlength\fheight{0.4\textwidth}
    \input{./tex_files/CM_80_3x4}
    \caption{3 \glspl{ap}, 4 antennas, 80 MHz}
    \label{fig:CM_80_3x4}
    \end{subfigure}
    %
    \hfill
    %
    \begin{subfigure}[t]{0.23\textwidth}
    \centering
    \setlength\fwidth{.7\textwidth}
    \setlength\fheight{0.4\textwidth}
    \input{./tex_files/CM_80_3x4}
    \caption{3 \glspl{ap}, 4 antennas, 80 MHz}
    \label{fig:CM_80_3x4}
    \end{subfigure}
            \setlength\abovecaptionskip{0.2cm}
    \centering
    \begin{subfigure}[t]{0.23\textwidth}
    \centering
    \setlength\fwidth{.7\textwidth}
    \setlength\fheight{0.4\textwidth}
    \input{./tex_files/CM_20_3x4}
    \caption{3 \glspl{ap}, 4 antennas, 20 MHz}
    \label{fig:CM_20_3x4}
    \end{subfigure}
    %
    \hfill
    %
    \begin{subfigure}[t]{0.23\textwidth}
    \centering
    \setlength\fwidth{.7\textwidth}
    \setlength\fheight{0.4\textwidth}
    \input{./tex_files/CM_80_3x4}
    \caption{3 \glspl{ap}, 4 antennas, 80 MHz}
    \label{fig:CM_80_3x4}
    \end{subfigure}
    %
    \hfill
    %
    \begin{subfigure}[t]{0.23\textwidth}
    \centering
    \setlength\fwidth{.7\textwidth}
    \setlength\fheight{0.4\textwidth}
    \input{./tex_files/CM_80_3x4}
    \caption{3 \glspl{ap}, 4 antennas, 80 MHz}
    \label{fig:CM_80_3x4}
    \end{subfigure}
    %
    \hfill
    %
    \begin{subfigure}[t]{0.23\textwidth}
    \centering
    \setlength\fwidth{.7\textwidth}
    \setlength\fheight{0.4\textwidth}
    \input{./tex_files/CM_80_3x4}
    \caption{3 \glspl{ap}, 4 antennas, 80 MHz}
    \label{fig:CM_80_3x4}
    \end{subfigure}
    \setlength\belowcaptionskip{-.5cm}
    \caption{Impact of frequency resolution and diversity.}
        \label{fig:t1ta_12_24}
\end{figure*}


==> tex_files/preamble.tex <==
\usepackage[acronyms,nonumberlist,nopostdot,nomain,nogroupskip]{glossaries}
\usepackage[numbers,sort&compress]{natbib}
\usepackage{xspace}
%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}
\usepackage{bm}
% \usepackage{url}
\usepackage[utf8]{inputenc}
\usepackage[table,xcdraw]{xcolor}
\usepackage{amsmath}
\usepackage{amssymb}
% \usepackage[numbers,sort&compress]{natbib}

\newcommand{\red}[1]{\begin{color}{red}#1\end{color}}





\usepackage[acronyms,nonumberlist,nopostdot,nomain,nogroupskip]{glossaries}
% \usepackage{tablefootnote}
\usepackage{booktabs}

\usepackage[acronyms,nonumberlist,nopostdot,nomain,nogroupskip]{glossaries}

\usepackage{tabularx}
\usepackage{graphicx}
\usepackage{epstopdf}

\usepackage{tikz}
\usepackage{arydshln}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\pgfplotsset{plot coordinates/math parser=false}
\newlength\fheight
\newlength\fwidth
\usetikzlibrary{plotmarks,patterns,decorations.pathreplacing,backgrounds,calc,arrows,arrows.meta,spy,matrix}
\usepgfplotslibrary{patchplots,groupplots,colorbrewer}
\usepackage{tikzscale}
% \usepackage[draft]{hyperref}

% externalize tikz plots - it should speed up compilation time
% https://tex.stackexchange.com/questions/1460/script-to-automate-externalizing-tikz-graphics
\newif\ifexttikz
\exttikzfalse

% Breaks with bizarre errors, could be that some options prevent externalization of tikz graphics
% https://tex.stackexchange.com/questions/450841/tikz-externalize-and-nicematrix-package?rq=1
% but it seems we don't use the options mentioned (nicematrix package,
%   and overlay or remember picture options

% \exttikztrue

\ifexttikz
	\usetikzlibrary{external}
	\tikzexternalize[prefix=figures/]
\fi


\usepackage{multirow}
% \usepackage{tkz-kiviat}

\renewcommand{\figurename}{Fig.}
%\renewcommand{\tablename}{Tab.}
\usepackage[font=footnotesize]{subcaption}
\usepackage[font=footnotesize]{caption}

\usepackage{mathtools}

% remove indent
% \usepackage{parskip}% http://ctan.org/pkg/parskip
% \setlength{\parindent}{0pt}

\usepackage{multirow}
\usepackage{url}
\usepackage{tabularx}
\usepackage{array}
\usepackage{multibib}
\newcites{methods}{References}

